Deep Chandra Observations of the z = 1.16 Relaxed, Cool-core Galaxy Cluster SPT-CL J2215-3537

Galaxy clusters serve as a unique and valuable laboratory for probing cosmological models and understanding astrophysics at the high-mass limit of structure formation. Clusters that are dynamically relaxed are especially useful targets of study because of their morphological and dynamical simplicity. However, at redshifts z > 1, very few such clusters have been identified. We present results from new Chandra observations of the cluster SPT-CL J2215-3537 (hereafter SPT J2215), at z = 1.16, the second most distant relaxed, cool-core cluster identified to date. We place constraints on the cluster's total mass profile and investigate its thermodynamic profiles, scaling relations (gas mass, average temperature, and X-ray luminosity), and metal enrichment, resolving the cool core and providing essential context for the massive starburst seen in its central galaxy. We contextualize the thermodynamic and cosmological properties of the cluster within a sample of well-studied, lower-redshift relaxed systems. In this way, SPT J2215 serves as a powerful high-redshift benchmark for understanding the formation of cool cores and the evolution of massive clusters of galaxies.

==> mnras-bib-defs.tex <==
%%% these were originally MNRAS-approved abbrevs

\def \aap {A\&A} % alternative A&A code
\def \aapr {A\&AR} % alternative A&AR
\def \aaps {A\&AS} % alternative A&AS
\def \statisci {Statis.\ Sci.} % statistical science
\def \physrep {Phys.\ Rep.} % physical review
\def \pre {Phys.\ Rev.\ E} % physical review E
\def \sjos {Scand.\ J.\ Statis.} % Scandinavian Journal of Statistics
\def \jrssb {J.\ Roy.\ Statist.\ Soc.\ B} % Journal of the Royal Statistical Society. Series B (Statistical Methodology)
\def \pan {Phys.\ Atom.\ Nucl.} % Physics of Atomic Nuclei
\def \epja {Eur.\ Phys.\ J.\ A} % European Physical Journal A
\def \epjc {Eur.\ Phys.\ J.\ C} % European Physical Journal C
\def \jcap {J.\ Cosmol.\ Astropart.\ Phys.} % Journal of Cosmology and Astro-Particle Physics
\def \ijmpd {Int.\ J.\ Mod.\ Phys.\ D} % international journal of modern physics D
\def \nar {New Astron.\ Rev.} % new astronomy review
\def \physscr{Phys.\ Scr.}      % Physica Scripta

% note: one of the macros below causes the dvips output to go crazy on the references page
% uncomment as necessary, at your own risk



% This is ASTROMNEMONIC.BIB, a bibliography database file that provides 
% mnmonics for journal names, which can be used in the `journal' field of 
% bibliography entries in databases for BibTeX.
% The abbreviations of the most popular Astronomical journal names in 
% this file are set out in 1993 MNRAS 160, 1. For the other journals,
% the abbreviations of the journal names in this file follow the rules of
% the International List of Periodical Title Word Abbreviations.
% From: Astronomy and Astrophysics Abstracts, 1990, Vol. 49A
% As coded in mnemonic.bib, by Sake J. Hogeveen.
%
% H. Ferguson 19 May 1993

\def \araa {ARA\&A}
% \def \afz {Afz}
\def \aj {AJ}
% \def \azh {AZh}
% \def \aa {A\&A}
% \def \aas {A\&AS}
\def \annstat {Ann.\ Stat.} % The Annals of Statistics
\def \aar {A\&AR}
\def \apj {ApJ}
\def \apjl {ApJ} %{ApJL}
\def \apjs {ApJS}
% \def \apss {Ap\&SS}
\def \asl {Adv.\ Sci.\ Lett.} % Advanced Science Letters
% \def \baas {BAAS}
% \def \jaa {JA\&A}
\def \mnras {MNRAS}
\def \nat {Nat}
\def \pasj {PASJ}
\def \pasp {PASP}
% \def \qjras {QJRAS}
\def \science {Sci}
% \def \sva {SvA}

% \def \aao {AAO Newsl.}
% \def \aavso {AAVSO Newsl.}
% \def \acta {Acta Astron.}
% \def \aaguv {Acta Astron.\ Geophys.\ Univ.\ Comenianae}
% \def \actastsin {Acta Astron.\ Sin.}
% \def \actapsin {Acta Astrophys.\ Sin.}
% \def \agg {Acta Geod.\ Geophys.}
% \def \ags {Acta Geophys.\ Sin.}
% \def \appsb {Acta Phys.\ Pol., Ser.\ B}
% \def \atash {Acta Tech.\ Acad.\ Sci.\ Hung.}
% \def \advp {Adv.\ Phys.}
% \def \advsr {Adv.\ Space Res.}
% \def \aip {AIP Conf.\ Proc.}
% \def \aavsob {Am.\ Assoc.\ Variable Star Obs.\ Bull.}
% \def \aavsoc {Am.\ Assoc.\ Variable Star Obs.\ Circ.}
% \def \amjp {Am.\ J.\ Phys.}
% \def \aatar {Anglo--Aust.\ Telesc., Annu.\ Rep.}
% \def \ag {Ann.\ Geophys.}
% \def \apl {Ann.\ Phys.\ (Leipzig)}
% \def \apny {Ann.\ Phys.\ (N.Y.)}
% \def \app {Ann.\ Phys.\ (Paris)}
% \def \ao {Appl.\ Opt.}
% \def \appl {Appl.\ Phys.\ Lett.}
% \def \apb {Appl.\ Phys., B}
% \def \as {Appl.\ Spectrosc.}
% \def \ahes {Arch.\ Hist.\ Exact Sci.}
% \def \archuk {Archeoastronomy (U.K.)}
% \def \asbts {Archenhold--Sternw.\ Berlin--Treptow, Sonderdr.}
% \def \asbtvs {Archenhold--Sternw.\ Berlin--Treptow, Vortr.\ Schr.}
% \def \aonaicnl {Arecibo Obs./NAIC, Newsl.}
% \def \artsat {Artif.\ Satell.}
% \def \aiisao {Astrofiz.\ Issled.\ Izv.\ Spets.\ Astrofiz.\ Obs.}
% \def \abco {Astron.\ Bull.\ (Carter Obs.)}
% \def \agas {Astron.\ Ges., Abstr.\ Ser.}
% \def \asther {Astron.\ Her.}
% \def \aiubc {Astron.\ Inst.\ Univ.\ Brno, Contrib.}
% \def \an {Astron.\ Nachr.}
% \def \astnow {Astron.\ Now}
% \def \astraum {Astron.\ Raumfahrt}
% \def \astriha {Astron.\ Rechen-Inst.Heidelb., Mitt., Ser.\ A}
% \def \astrihb {Astron.\ Rechen-Inst.Heidelb., Mitt., Ser.\ B}
% \def \astschu {Astron.\ Sch.}
% \def \asttid {Astron.\ Tidsskr.}
% \def \asttsir {Astron.\ Tsirk.}
% \def \astvest {Astron.\ Vestn.}
% \def \astuai {Astronomia UAI}
% \def \astie {Astronomie}
% \def \asty {Astronomy}
% \def \aplc {Astrophys.\ Lett.\ Commun.}
% \def \ap {Astrophysics}
% \def \aanlsor {Atti Accad.\ Naz.\ Lincei, Ser.\ Ottava, Rend.}
% \def \ajast {Aust.\ J.\ Astron.}
% \def \ajp {Aust.\ J.\ Phys.}
% \def \bavm {BAV Mitt.}
% \def \bavr {BAV Rundbrief}
% \def \bbsag {BBSAG Bull.}
% \def \bestarnl {Be Star Newsl.}
% \def \bildw {Bild Wiss.}
% \def \bipm {BIPM Circ.\ T}
% \def \boaumkt {Biul.\ Obs.\ Astron.\ Uniw.\ M.\ Kopernika Toruniu}
% \def \boe {Bol.\ Obs.\ Ebro}
% \def \broa {Bol.\ ROA}
% \def \blm {Boundary-Layer Meteorol.}
% \def \boop {Boyden Obs., Occas.\ Publ.}
% \def \bastac {Br.\ Astron.\ Assoc.\ Circ.}
% \def \bjp {Bulg.\ J.\ Phys.}
% \def \baps {Bull.\ Am.\ Phys.\ Soc.}
% \def \bafoev {Bull.\ Assoc.\ Fr.\ Obs.\ Etoiles Variables}
% \def \bastic {Bull.\ Astron.\ Inst.\ Czech.}
% \def \basi {Bull.\ Astron.\ Soc.\ India}
% \def \bcao {Bull.\ Crimean Astrophys.\ Obs.}
% \def \bgsi {Bull.\ Geogr.\ Surv.\ Inst.}
% \def \bicds {Bull.\ Inf.\ Cent.\ Donn\'ees Stellaires}
% \def \boab {Bull.\ Obs.\ Astron.\ Belgr.}
% \def \crassgvs {C.\ R.\ Acad.\ Sci., S\'er.\ G\'en., Vie Sci.}
% \def \crassii {C.\ R.\ Acad.\ Sci., II}
% \def \cjp {Can.\ J.\ Phys.}
% \def \cm {Celest.\ Mech.}
% \def \cassos {Cent.\ Astron.\ Sci.\ Spat., Obs.\ Sol.}
% \def \cent {Centaurus}
% \def \cpl {Chem.\ Phys.\ Lett.}
% \def \chinaa {Chin.\ Astron.\ Astrophys.}
% \def \chinp {Chin.\ Phys.}
% \def \chinpl {Chin.\ Phys.\ Lett.}
% \def \ciel {Ciel}
% \def \cielt {Ciel Terre}
% \def \ccotl {Circ.\ Czech.\ Obs.\ Time Lattiude}
% \def \cinf {Circ.\ Inf.}
% \def \ctls {Circ.\ Time Latitude Serv.}
% \def \cqg {Classical Quantum Gravity}
% \def \cast {Comments Astrophys.}
% \def \cnpp {Comments Nucl.\ Part.\ Phys.}
% \def \cppcf {Comments Plasma Phys.\ Controlled Fusion}
% \def \cfsua {Commun.\ Fac.\ Sci.\ Univ.\ Ankara, Ser.\ A2, A3}
% \def \cko {Commun.\ Konkoly Obs.}
% \def \cmp {Commun.\ Math.\ Phys.}
% \def \culo {Commun.\ Univ.\ Lond.\ Obs.}
% \def \comp {Comput.\ Phys.}
\def \compcom {Comput.\ Phys.\ Commun.}
% \def \cp {Contemp.\ Phys.}
% \def \caosp {Contrib.\ Astron.\ Obs.\ Skalnat\'e Pleso}
% \def \cap {Contrib.\ Atmos.\ Phys.}
% \def \cdaut {Contrib.\ Dep.\ Astron., Univ.\ Tokyo}
% \def \clo {Contrib.\ Lick Obs.}
% \def \cncopb {Contrib.\ Nicholas Copernicus Obs.\ Planetarium Brno}
% \def \cnjro {Contrib.\ Nizamiah Japal-Rangapur Obs.}
% \def \cpp {Contrib.\ Plasma Phys.}
% \def \cvvo {Contrib.\ Van Vleck Obs.}
% \def \cr {Cosmic Res.}
% \def \cryo {Cryogenics}
% \def \czjp {Czech.\ J.\ Phys., Sect.\ B}
% \def \drho {Data Rep.\ Hydrogr.\ Obs., Ser.\ Astron.\ Geod.}
% \def \dgkbawb {Dtsch.\ Geod.\ Komm.\ Bayer.\ Akad.\ Wiss., Reihe B}
% \def \dgkbawc {Dtsch.\ Geod.\ Komm.\ Bayer.\ Akad.\ Wiss., Reihe C}
% \def \dgkbawe {Dtsch.\ Geod.\ Komm.\ Bayer.\ Akad.\ Wiss., Reihe E}
% \def \epsl {Earth Planet.\ Sci.\ Lett.}
% \def \erb {Earth Rotation Bull.}
% \def \emp {Earth, Moon, Planets}
% \def \esrev {Earth--Sci.\ Rev.}
% \def \esab {ESA Bull.}
% \def \esaiuenl {ESA IUE Newsl.}
% \def \esaj {ESA J.}
% \def \esoar {ESO Ann.\ Rep.}
% \def \ejp {Eur.\ J.\ Phys.}
% \def \epl {Europhys.\ Lett.}
% \def \epn {Europhys.\ News}
% \def \expast {Exp.\ Astron.}
% \def \fiz {Fizika}
% \def \fortp {Fortschr.\ Phys.}
% \def \fp {Found.\ Phys.}
% \def \funcp {Fundam.\ Cosmic Phys.}
% \def \gaab {G.~A.A.B.}
% \def \gast {G.\ Astron.}
% \def \gem {Gemini}
% \def \grg {Gen.\ Relativ.\ Gravitation}
\def \gca {Geochim.\ Cosmochim.\ Acta}
% \def \ga {Geomagn.\ Aehron.}
% \def \gafd {Geophys.\ Astrophys.\ Fluid Dyn.}
% \def \gj {Geophys.\ J.}
% \def \grl {Geophys.\ Res.\ Lett.}
% \def \geo {Geophysics}
% \def \geos {GEOS Circ.}
% \def \gbg {Gerlands Beitr.\ Geophys.}
% \def \heav {Heavens}
% \def \hpa {Helv.\ Phys.\ Acta}
% \def \hepnp {High Energ.\ Phys.\ Nucl.\ Phys.}
% \def \hob {Hvar Obs.\ Bull.}
% \def \hi {Hyperfine Interact.}
% \def \iappp {I.A.P.P.P.\ Commun.}
% \def \iauc {IAU Circ.}
% \def \iauib {IAU Inf.\ Bull.}
% \def \icarus {Icarus}
% \def \i3etm {IEEE Trans.\ Magn.}
% \def \i3etns {IEEE Trans.\ Nucl.\ Sci.}
% \def \i3etps {IEEE Trans.\ Plasma Sci.}
% \def \iersbb {IERS Bull.\ B}
% \def \iersba {IERS Bull.--A}
% \def \ijpap {Indian J.\ Pure Appl.\ Phys.}
% \def \ijrsp {Indian J.\ Radio Space Phys.}
% \def \ibvs {Inf.\ Bull.\ Variable Stars}
% \def \iaatub {Inst.\ Astron.\ Astrophys.\ Tech.\ Univ.\ Berlin, Mitt.}
% \def \iag {Inst.\ Astron.\ Geod., Univ.\ Madr., Publ.}
% \def \ia {Inst.\ Astron., Univ.\ Camb., Annu.\ Rep.}
% \def \icq {Int.\ Comet Q.}
% \def \ijimw {Int.\ J.\ Infrared Millimeter Waves}
% \def \ijmp {Int.\ J.\ Mod.\ Phys.\ A}
% \def \ijtp {Int.\ J.\ Theor.\ Phys.}
% \def \ip {Inverse Probl.}
% \def \iastj {Ir.\ Astron.\ J.}
% \def \iris {IRIS Bull.\ A}
% \def \iskz {Issled.\ Solntsa Krasnykh Zvezd}
% \def \intsa {Itogi Nauki Tekh., Ser.\ Astron.}
% \def \intsppk {Itogi NAuki Tekh., Ser.\ Plazmennye Protsessy Kosmose}
% \def \iaoe {Izv.\ Astron.\ Obs.\ Ehngel'gardt.}
% \def \ikao {Izv.\ Krym.\ Astrofiz.\ Obs.}
% \def \ivuzr {Izv.\ Vyssch.\ Uchebn.\ Zaved., Radiofiz.}
% \def \jasa {J.\ Acoust.\ Soc.\ Am.}
% \def \jaavso {J.\ Am.\ Assoc.\ Variable Star Obs.}
% \def \jam {J.\ Appl.\ Meteorol.}
% \def \jap {J.\ Appl.\ Phys.}
% \def \jastf {J.\ Astron.\ Fr.}
% \def \japast {J.\ Astrophys.\ Astron.}
% \def \jas {J.\ Atmos.\ Sci.}
\def \jasa {J.\ Am.\ Stat.\ Assoc.} % Journal of the American Statistical Association
% \def \jatp {J.\ Atmos.\ Terr.\ Phys.}
% \def \jbasta {J.\ Br.\ Astron.\ Assoc.}
% \def \jbis {J.\ Br.\ Interplanet.\ Soc.}
% \def \jcp {J.\ Chem.\ Phys.}
\def \jcgs {J.\ Comput.\ Graph.\ Stat.} % Journal of Computational and Graphical Statistics
% \def \jcomp {J.\ Comp.\ Phys.}
% \def \jel {J.\ Electrostat.}
% \def \jfseu {J.\ Fac Sci., Ege Univ., Ser.\ A}
% \def \jfm {J.\ Fluid Mech.}
% \def \jgr {J.\ Geophys.\ Res.}
% \def \jhast {J.\ Hist.\ Astron.}
% \def \jms {J.\ Mater.\ Sci.}
% \def \jmp {J.\ Math.\ Phys.}
% \def \jmo {J.\ Mod.\ Opt.}
% \def \jop {J.\ Opt.\ (Paris)}
% \def \josaa {J.\ Opt.\ Soc.\ Am.\ A}
% \def \josab {J.\ Opt.\ Soc.\ Am.\ B}
% \def \jp {J.\ Phys.}
% \def \jpa {J.\ Phys.\ A}
% \def \jpb {J.\ Phys.\ B}
% \def \jpd {J.\ Phys.\ D}
% \def \jpe {J.\ Phys.\ E}
% \def \jpg {J.\ Phys.\ G}
% \def \jpsj {J.\ Phys.\ Soc.\ Jpn.}
% \def \jpp {J.\ Plasma Phys.}
% \def \jqsrt {J.\ Quant.\ Spectrosc.\ Radiat.\ Transfer}
% \def \jrasc {J.\ R.\ Astron.\ Soc.\ Can.}
% \def \jsp {J.\ Stat.\ Phys.}
\def \jspi {J.\ Stat.\ Plan.\ Inference} % Journal of Statistical Planning and Inference
% \def \jvst {J.\ Vac.\ Sci.\ Technol., A}
% \def \jetpl {JETP Lett.}
% \def \jhatd {Johns Hopkins APL Tech.\ Dig.}
% \def \jjap1 {Jpn.\ J.\ Appl.\ Phys., Part 1}
% \def \jjap2 {Jpn.\ J.\ Appl.\ Phys., Part 2}
% \def \kai {Kapteyn Astron.\ Inst., Annu.\ Rep.}
% \def \kexto {Kexue Tongbao}
% \def \kfnt {Kinematika Fiz.\ Nebesn.\ Tel}
% \def \kob {Kodaikanal Obs.\ Bull.}
% \def \kt {Komet.\ Tsirk.}
% \def \ki {Kosm.\ Issled.}
% \def \koz {Kozmos}
% \def \kpm {KPM}
% \def \lo {Laser Optoelektron.}
% \def \latc {Latitude Circ.}
% \def \lest {LEST Found., Annu.\ Rep.}
% \def \lmp {Lett.\ Math.\ Phys.}
% \def \lob {Lick Obs.\ Bull.}
% \def \mg {Manuscr.\ Geod.}
% \def \ml {Mater.\ Lett.}
% \def \mrb {Mater.\ Res.\ Bull.}
% \def \mfs {Mem.\ Fac.\ Sci., Kyoto Univ., Ser.\ Phys., Astrophys., Geophys., Chem.}
% \def \msai {Mem.\ Soc.\ Astron.\ Ital.}
% \def \merc {Mercury}
% \def \mess {Messenger}
% \def \met {Meteoritics}
% \def \metka {Meteoritika}
% \def \metro {Metrologica}
% \def \mpb {Minor Planet Bull.}
% \def \mpc {Minor Planet Circ.}
% \def \masbt {Mitt.\ Archenold--Sternw.\ Berlin Treptow}
% \def \mag {Mitt.\ Astron.\ Ges.}
% \def \mlotud {Mitt.\ Lohrmann--Obs., Tech.\ Univ.\ Dresden}
% \def \mss {Mitt.\ Sternw.\ Sonneberg}
% \def \mvs {Mitt.\ Ver{\a}nderliche Sterne"}
% \def \mzpe {Mitt.\ Zentralinst.\ Phys.\ Erde}
% \def \mpla {Mod.\ Phys.\ Lett.\ A}
% \def \mnassa {Mon.\ Notes Astron.\ Soc.\ S.\ Afr.}
% \def \nint {Nablyud.\ Iskusstv.\ Nebesn.\ Tel.}
% \def \nogb {Nachr.\ Olbers--Ges.\ Bremen}
% \def \naoj {Natl.\ Astron.\ Obs.\ (Jpn.), Repr.}
% \def \ng {Natl.\ Geogr.}
% \def \nraoa {Natl.\ Radio Astron.\ Obs., Repr., Ser.\ A}
% \def \nraob {Natl.\ Radio Astron.\ Obs., Repr., Ser.\ B}
% \def \natwis {Naturwissenschaften}
% \def \ni {Nauchn.\ Inf.}
% \def \nlasny {News Lett.\ Astron.\ Soc.\ N.Y.}
% \def \nrodaour {Nizamiah Rangapur Obs.\ Dep.\ Astron., Osmania Univ., Repr.}
% \def \nraow {NRAO Workshop}
% \def \nimpra {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ A}
% \def \nimprb {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ B}
\def \npa {Nucl.\ Phys.\ A}
% \def \npb {Nucl.\ Phys.\ B, Part.\ Phys.}
% \def \nca {Nuovo Cimento A}
% \def \ncb {Nuovo Cimento B}
% \def \ncc {Nuovo Cimento C}
% \def \ot {Obs.\ Trav.}
% \def \obs {Observatory}
% \def \onl {Occultation Newsl.}
% \def \ozvp {{\O}sterr.\ Z.\ Vermessungswes.\ Photogramm."}
% \def \oc {Opt.\ Commun.}
% \def \oe {Opt.\ Eng.}
% \def \olt {Opt.\ Laser Technol.}
% \def \ol {Opt.\ Lett.}
% \def \on {Opt.\ News}
% \def \os {Opt.\ Spectrosc.}
% \def \optik {Optik}
% \def \ofeb {Origins Life Evol.\ Biosphere}
% \def \orion {Orion}
% \def \orione {Orione}
% \def \oac {Oss.\ Astrofis.\ Catania, Pubbl.}
% \def \pz {Perem.\ Zvezdy}
% \def \pb {Phys.\ Bl.}
% \def \pcm {Phys.\ Chem.\ Miner.}
% \def \pfa {Phys.\ Fluids, A}
% \def \pfb {Phys.\ Fluids, B}
% \def \pla {Phys.\ Lett.\ A}
\def \plb {Phys.\ Lett.\ B}
% \def \pr {Phys.\ Rep.}
% \def \pra {Phys.\ Rev.\ A}
% \def \prb {Phys.\ Rev.\ B}
\def \prc {Phys.\ Rev.\ C}
\def \prd {Phys.\ Rev.\ D}
\def \prl {Phys.\ Rev.\ Lett.}
% \def \ps {Phys.\ Scr.}
% \def \ptch {Phys.\ Teach.}
% \def \ptod {Phys.\ Today}
% \def \pha {Physica A}
% \def \phb {Physica B}
% \def \phd {Physica D}
% \def \paz {Pis'ma Astron.\ Zh.}
% \def \pss {Planet.\ Space Sci.}
% \def \ppcf {Plasma Phys.\ Controlled Fusion}
% \def \pa {Postepy Astron.}
% \def \pram {Pram\~{a}na}
% \def \pri {Priroda}
\def \pasa {Proc.\ Astron.\ Soc.\ Aust.}
% \def \pi3e {Proc.\ IEEE}
% \def \prsl {Proc.\ R.\ Soc.\ London, Ser.\ A}
% \def \posp {Proceedings of SPIE}
% \def \past {Prog.\ Astron.}
% \def \ptp {Prog.\ Theor.\ Phys.}
% \def \paicas {Publ.\ Astron.\ Inst.\ Czech.\ Acad.\ Sci.}
% \def \pbao {Publ.\ Beijing Astron.\ Obs.}
% \def \pdaub {Publ.\ Dep.\ Astron., Univ.\ Beogr.}
% \def \pdao {Publ.\ Dom.\ Astrophys.\ Obs.}
% \def \pnlaoj {Publ.\ Natl.\ Astron.\ Obs.\ Jpn.}
% \def \ppmo {Publ.\ Purple Mt.\ Obs.}
% \def \psao {Publ.\ Shaanxi Astron.\ Obs.}
% \def \pscds {Publ.\ Sp\'ec.\ Cent.\ Donn\'ees Stellaires}
% \def \pyo {Publ.\ Yunnan Obs.}
% \def \pag {Pure Appl.\ Geophys.}
% \def \qbsa {Q.\ Bull.\ Sol.\ Act.}
% \def \rad {Radiant}
% \def \rsci {Radio Sci.}
% \def \reche {Recherche}
% \def \rpp {Rep.\ Prog.\ Phys.}
% \def \ra {Rev.\ Astron.}
% \def \rg {Rev.\ Geophys.}
% \def \rmf {Rev.\ Mex.\ Fis.}
% \def \rmp {Rev.\ Mod.\ Phys.}
% \def \rrp {Rev.\ Roum.\ Phys.}
% \def \rsi {Rev.\ Sci.\ Instrum.}
% \def \rnc {Riv.\ Nuovo Cimento}
% \def \rh {\v{R}\'{\i}\v{s}e hv\v{e}zd}
% \def \saaoar {S.\ Afr.\ Astron.\ Obs., Annu.\ Rep.}
% \def \saaoc {S.\ Afr.\ Astron.\ Obs., Circ.}
% \def \saaon {SAAO Newsl.}
% \def \sciam {Sci.\ Am.}
% \def \scch {Sci.\ China, Ser.\ A}
% \def \srtu {Sci.\ Rep.\ T\^{o}hoku Univ., Eighth Ser.}
% \def \sc {Science}
% \def \sar {Sendai Astron.\ Rap.}
% \def \st {Sidereal Times}
% \def \sky {Sky Telesc.}
% \def \sbaavso {Sol.\ Bull.\ (AAVSO)}
% \def \se {Sol.\ Energy}
% \def \sp {Sol.\ Phys.}
% \def \srd {Sol.\ Radio Data}
% \def \ssres {Sol.\ Syst.\ Res.}
% \def \sdb {Soln.\ Dannye, Byull.}
% \def \sonne {Sonne}
% \def \sbo {Soobshch.\ Byurak.\ Obs.}
% \def \ssao {Soobshch.\ Spets.\ Astrofiz.\ Obs.}
% \def \sost {South.\ Stars}
% \def \sal {Sov.\ Astron.\ Lett.}
% \def \sjot {Sov.\ J.\ Opt.\ Technol.}
% \def \spd {Sov.\ Phys.\ -- Dokl.}
% \def \spj {Sov.\ Phys.\ -- JETP}
% \def \spu {Sov.\ Phys.\ -- Usp.}
% \def \space {Space}
\def \ssr {Space Sci.\ Rev.}
\def \statsin {Stat.\ Sin.} % Statistica Sinica
% \def \stsi {Space Telesc.\ Sci.\ Inst., Newsl.}
% \def \sf {Spaceflight}
% \def \sterne {Sterne}
% \def \sw {Sterne Weltraum}
% \def \sb {Sternenbote}
% \def \strlast {Strolling Astron.}
% \def \sgg {Stud.\ Geophys.\ Geod.}
% \def \taot {Tartu Astrof{\u}{\"u}s.\ Obs.\ Teated"}
% \def \tect {Tectonophysics}
% \def \tellus {Tellus, Ser.\ A}
% \def \tmf {Teor.\ Mat.\ Fiz.}
% \def \tp {Theor.\ Pap.}
% \def \tsb {Time Serv.\ Bull.}
% \def \tmnr {Tokyo Meteor Network Rep.}
% \def \tai {Tsirk.\ Astron.\ Inst.\ (Tashkent)}
% \def \ufz {Ukr.\ Fiz.\ Zh.}
% \def \ucla {Universe Classroom}
% \def \uao {Upps.\ Astron.\ Obs., Rep.}
% \def \urania {Urania}
% \def \usnoc {U.S.\ Nav.\ Obs., Circ.}
% \def \usnos4 {U.S.\ Nav.\ Obs., Ser.\ 4}
% \def \ufn {Usp.\ Fiz.\ Nauk}
% \def \vsb {Variable Star Bull.}
% \def \vasiona {Vasiona}
% \def \varih {Ver{\o}ff.\ Astron.\ Rechen--Inst.\ Heidelb."}
% \def \vzpe {Ver{\o}ff.\ Zentralinst.\ Phys.\ Erde"}
% \def \vesmir {Vesm\'{\i}r}
% \def \vansssr {Vestn.\ Akad.\ Nauk SSSR}
% \def \vku {Vestn.\ Kiev.\ Univ., Astron.}
% \def \va {Vistas Astron.}
% \def \wgn {WGN}
% \def \wztud {Wiss.\ Z.\ Tech.\ Univ.\ Dresden}
% \def \yama {Yamamoto Circ.}
% \def \zamp {Z.\ Angew.\ Math.\ Phys.}
% \def \zna {Z.\ Naturforsch., A}
% \def \zpa {Z.\ Phys., A}
% \def \zpc {Z.\ Phys., C}
% \def \zv {Zemlya Vselennaya}
% \def \zenit {Zenit}
% \def \zetf {Zh.\ Ehksp.\ Teor.\ Fiz.}

